Criticality of $\text{AC}^0$ formulae

Rossman [In $\textit{Proc. $34$th Comput. Complexity Conf.}$, 2019] introduced the notion of $\textit{criticality}$. The criticality of a Boolean function $f : \{0,1\}^n \to \{0,1\}$ is the minimum $\lambda \geq 1$ such that for all positive integers $t$, \[ \Pr_{\rho \sim \mathcal{R}_p}\left[\text{DT}_{\text{depth}}(f|_{\rho}) \geq t\right] \leq (p\lambda)^t. \] H\"astad's celebrated switching lemma shows that the criticality of any $k$-DNF is at most $O(k)$. Subsequent improvements to correlation bounds of $\text{AC}^0$-circuits against parity showed that the criticality of any $\text{AC}^0$-$\textit{circuit}$ of size $S$ and depth $d+1$ is at most $O(\log S)^d$ and any $\textit{regular}$ $\text{AC}^0$-$\textit{formula}$ of size $S$ and depth $d+1$ is at most $O\left(\frac1d \cdot \log S\right)^d$. We strengthen these results by showing that the criticality of $\textit{any}$ $\text{AC}^0$-formula (not necessarily regular) of size $S$ and depth $d+1$ is at most $O\left(\frac1d\cdot {\log S}\right)^d$, resolving a conjecture due to Rossman. This result also implies Rossman's optimal lower bound on the size of any depth-$d$ $\text{AC}^0$-formula computing parity [$\textit{Comput. Complexity, 27(2):209--223, 2018.}$]. Our result implies tight correlation bounds against parity, tight Fourier concentration results and improved $\#$SAT algorithm for $\text{AC}^0$-formulae.

==> macros.tex <==

%%%%%%%%%%%%%%%%%%
\newcommand{\CDT}{\operatorname{CDT}}
\newcommand{\dom}{\operatorname{Dom}}
\newcommand{\stars}{\operatorname{stars}}
\newcommand{\calR}{\mathcal{R}}
%%%%%%%%%%%%%%%%%
%macros
%names
\newcommand{\demorgan}{De-Morgan\ }
\newcommand{\hastad}{H\aa stad}

%functions%
\newcommand{\sym}{\mathrm{SYM}}
\newcommand{\thr}{\mathrm{LTF}}
\newcommand{\maj}{\mathrm{MAJ}}
\newcommand{\IN}{\mathrm{IN}}
\newcommand{\AND}{\mathrm{AND}}
\newcommand{\OR}{\mathrm{OR}}
\newcommand{\MOD}{\mathrm{MOD}}
\newcommand{\xor}{\oplus}

%shortcuts%
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\setcond}[2]{\left\{#1\: \middle|\: #2\right\}}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\cgeq}{\succcurlyeq}
\newcommand{\cleq}{\preccurlyeq}

%probability
\newcommand{\prob}[2]{\Pr_{#1}\left[#2\right]}
\newcommand{\E}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\Ex}[2]{\underset{#1}{\mathbb{E}} \left[ #2 \right]}


%boolean functions and cubes
\newcommand{\zo}{\{0,1\}}
\newcommand{\pmone}{\{-1,1\}}
\newcommand{\bool}[1]{\zo^{#1} \rightarrow \cube{}}
\newcommand{\fbool}[1]{\pmone^{#1} \rightarrow \fcube{}}

%Brackets%
\newcommand{\bra}[1]{\left\{#1\right\}}
\newcommand{\sbra}[1]{\left[#1\right]}
\newcommand{\abra}[1]{\left\langle#1\right\rangle}
\newcommand{\cbra}[1]{\left(#1\right)}

%Symbols%
\newcommand{\IF}{\mathrm{if}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\p}{\mathcal{P}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}



%caligraphic symbols
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\rhotilde}{\Tilde{\rho}}
\newcommand{\dist}{\calR(\tilde{p})}
\newcommand{\pivots}{\operatorname{Pivots}}

%asymptotic notation
\newcommand{\bigo}[1]{O\left(#1\right)}
\newcommand{\smallo}[1]{o\left(#1\right)}

\newcommand{\ie}{\emph{i.e.}}

%%environments
%\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
%\newtheorem*{theorem*}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem*{lemma*}{Lemma}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{claim}[theorem]{Claim}
%\newtheorem*{claim*}{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{conjecture}{Conjecture}
%\newtheorem*{conjecture*}{Conjecture}
\newtheorem{question}{Question}
%\newtheorem*{question*}{Question}
%\newtheorem*{answer*}{Answer}
%%commands%
